The RESET and MARC Techniques, with Application to Multiserver-Job Analysis

Multiserver-job (MSJ) systems, where jobs need to run concurrently across many servers, are increasingly common in practice. The default service ordering in many settings is First-Come First-Served (FCFS) service. Virtually all theoretical work on MSJ FCFS models focuses on characterizing the stability region, with almost nothing known about mean response time. We derive the first explicit characterization of mean response time in the MSJ FCFS system. Our formula characterizes mean response time up to an additive constant, which becomes negligible as arrival rate approaches throughput, and allows for general phase-type job durations. We derive our result by utilizing two key techniques: REduction to Saturated for Expected Time (RESET) and MArkovian Relative Completions (MARC). Using our novel RESET technique, we reduce the problem of characterizing mean response time in the MSJ FCFS system to an M/M/1 with Markovian service rate (MMSR). The Markov chain controlling the service rate is based on the saturated system, a simpler closed system which is far more analytically tractable. Unfortunately, the MMSR has no explicit characterization of mean response time. We therefore use our novel MARC technique to give the first explicit characterization of mean response time in the MMSR, again up to constant additive error. We specifically introduce the concept of "relative completions," which is the cornerstone of our MARC technique.

==> draft-of-proofs.tex <==




\isaac{Outline up to here}

\section{Setting: Markov Modulated Completions Queue.}

Jobs arrive according to a Poisson process with rate $\lambda$.

The completion process is controlled by a Markov chain $\{Y\}$, whose state at time $t$ is $Y(t)$.
We write $Y$ to represent the random variable denoting
the steady state of the chain $\{Y\}$.
Let $y$ represent a generic state of the Markov chain.
A state of the overall system is
$(y, q)$, where $q$ is the number of jobs in the queue.
The steady state of the overall system is
$(Y, Q)$.
When the Markov chain $\{Y\}$ is in state $y$,
at rate $\mu_{y, y', a}$
it transitions to state $y'$
while completing $a \le 1$ jobs.

\begin{definition}
    Let $r(y)$ represent the instantaneous completion rate
    in state $y$:
    \begin{align*}
        r(y) = \sum_{y'} \mu_{y,y',1}.
    \end{align*}
\end{definition}

\begin{definition}
    Let $\pi(y)$ represent the steady state probability
    of $\{Y\}$ being in state $y$:
    \begin{align*}
        \pi(y) = P(Y = y).
    \end{align*}
\end{definition}

\begin{definition}
    Let $\rbar$ represent the time-average completion rate:
    \begin{align*}
        \rbar = E[r(Y)]
    \end{align*}
\end{definition}

We know define the \emph{relative value function} $g(y)$
to be the transient additional number of completions
expected to occur starting from state $y$,
compared to the time-average completion rate.

\begin{definition}
    Let $g(y)$ denote the relative value function:
    \begin{align*}
        g(y) = \int_0^\infty E[ r(Y(t)) - \rbar | Y(0) = y] dt.
    \end{align*}
    \isaac{I think that the limit should be outside the integral} \\
    Let $C_t$ denote the number that occur between times $0$ and $t$. Then an equivalent definition of $g(y)$ is:
    \begin{align*}
        g(y) = E[\lim_{t \to \infty} C_t - \rbar t | Y(0) = y]
    \end{align*}
\end{definition}
\isaac{Need to prove $g(y)$ is well defined - use $\{Y\}$ is finite-state.}

Note that $E[g(Y)] = 0$, because $Y(s) = Y$ for all $s$, and so $E[r(Y(s))] = \rbar$.

\isaac{A useful set of linear equations for solving for $g(y)$, up to an additive constant:}
\begin{align*}
    \isaac{\qquad g(y) = \frac{r(y) - \rbar}{\mu(y)} + \sum_{y'} g(y') \frac{\mu_{y,y'}}{\mu(y)} \qquad}
\end{align*}
Next, let us define the completion-average state of the Markov chain - the average state which occurs just after a completion.
\begin{definition}
    Let $Y^e$ denote the completion-average state of $\{Y\}$:
    \begin{align*}
        P(Y^e = y') = C \sum_y (\pi_y r(y)) \frac{\mu_{y,y',1}}{r(y)}
        = C \sum_y \pi_y \mu_{y,y',1}
    \end{align*}
    where $C$ is a normalization constant.
    In fact, $C = \frac{1}{\rbar}$, so this expression is actually:
    \begin{align*}
        P(Y^e = y')
        = \frac{1}{\rbar} \sum_y \pi_y \mu_{y,y',1}
    \end{align*}
\end{definition}


\begin{definition}
    Let $G$ denote the generator of the overall Markov chain $\{(Q, Y)\}$.
    For any function $z(q, y)$,
    \begin{align*}
        G z(q, y) = \lim_{s \to 0} \frac{1}{s} E[z(Y(s), Q(s)) - z(y,q)|Y(0) = y, Q(0)=q]
    \end{align*}
\end{definition}
\isaac{For example, $G g(y) = \rbar - r(y)$.}


\isaac{TODO: Same argument, but for MSJ system, not MMCQ. Should transfer nearly immediately, no busy periods needed.}
\section{MSJ asymptotics match MMCQ}
We want to show that
the MSJ model has the same asymptotic queue length as the MMCQ.

MSJ model definition:
A state consists of a tuple $(y, q)$,
where $y$ is a list of up to $k$ job types,
and $q$ is a number of jobs.
If $q > 0$, $y$ has exactly $k$ jobs.

The completion rate is only dependent on $y$, not on $q$.
When a job completes, if $q>0$, a job is removed from $y$, a new job is sampled, and $q$ is decremented.
Otherwise, no new job is sampled.
If a job arrives when $|y| < k$, a new job is added to $y$.
Otherwise, $q$ is incremented.

We will show that
the behavior of a MSJ system is very similar to the corresponding MMCQ system, called the saturated system.
The saturated system is defined by considering a Markov chain over the states $y$ where $|y| = k$.
Think of this system as always adding a new job to $y$ whenever a job completes.
The completion process in the saturated system simply consists of this Markov chain's
completion process.

We will show that
\begin{align*}
    E[Q^{MSJ}] = E[Q^{MMCQ}] + O(1) = \frac{E[g(Y^e)] + 1}{1-\rho} + O(1)
\end{align*}
We will make use of a similar potential function as in the MMCQ proof:
\begin{align*}
    f^{MSJ}(q, y)=\frac{1}{2} (q-g^{MSJ}(y))^2
\end{align*}
where $g^{MSJ}$ is identical to $g^{MMCQ}$
on saturated $y$, and arbitrarily set to 0
on all unsaturated $y$ ($|y| < k$).
The value of $g^{MSJ}$ on unsaturated $y$ will turn out to be irrelevant.

Let us examine $G^{MSJ} f^{MSJ}(q, y)$.

\begin{align*}
    G^{MSJ} f^{MSJ}(q, y) = \begin{cases}
        G^{MMCQ} f^{MSJ}(q, y) & q > 0 \\
        0 & |y| < k-1 \\
        (\text{arrivals only}) & |y| = k-1 \\
        (\text{anything}) & |y| = k, q = 0
    \end{cases}
\end{align*}
Note that this is identical to $G^{MMCQ} f^{MSJ}(q, y)$,
except for differing by a constant in states where $q=0$.
We will show that $P(Q^{MSJ} = 0) = O(1-\rho)$.
We will therefore argue that
\begin{align*}
    0 = E[G^{MSJ} f^{MSJ}(Q^{MSJ}, Y^{MSJ})] = (\lambda - \rbar)E[Q^{MSJ}] - E[c(Y^{MSJ})] + O(1-\rho)
\end{align*}
Moreover, we will exhibit a coupling under which $P(Y^{MSJ} \neq Y^{MMCQ}) = O(1-\rho)$.
We will therefore conclude that 
\begin{align*}
    0 &= G^{MSJ} f^{MSJ}(Q^{MSJ}, Y^{MSJ}) = (\lambda - \rbar)E[Q^{MSJ}] - E[c(Y^{MMCQ})] + O(1-\rho) \\
    E[Q^{MSJ}] &= \frac{E[c(Y^{MMCQ})]}{\rbar - \lambda} + O(1) = \frac{1+E[g(Y^e)]}{1-\rho} + O(1)
\end{align*}
It therefore suffices to show that $P(Q^{MSJ} = 0) = O(1-\rho)$ and $P(Y^{MSJ} \neq Y^{MMCQ}) = O(1-\rho)$.

Let us start by defining our coupling:

The two systems have arrivals at the same times. If $y^{MSJ} = y^{MMCQ}$,
the two systems have the same completions at the same times (and the same $y$ transitions in general \yige{i.e., if $q > 0$}). If $y^{MSJ} \neq y^{MMCQ}$,
completions (and $y$ transitions) are independent in the two systems.

We wish to show two properties of the MSJ system, for any $\epsilon \le \rho < 1$:
\begin{enumerate}
\item Property 1: $P(Q^{MSJ}=0) = O(1-\rho)$
\item Property 2: $P(Y^{MSJ} \neq Y^{MMCQ}) = O(1-\rho)$.
\end{enumerate}
We will show that property 2 holds under the coupling specified above.

We will prove these two properties by building on two more basic facts:
\begin{enumerate}
    \item Fact 1: From any joint MSJ, MMCQ state, under the coupling above,
    the expected time until $y^{MSJ}=y^{MMCQ}$, $q^{MSJ} \ge k+1$, and $q^{MMCQ} \ge k+1$
    is at most $M_1$ for some $M_1$ independent of $\rho$ and initial joint states,
    given that $\epsilon \le \rho < 1$.
    \item Fact 2: From any joint MSJ, MMCQ state such that
    $y^{MSJ}=y^{MMCQ}$, $q^{MSJ} \ge k+1$, and $q^{MMCQ} \ge k+1$, the expected time until $q^{MSJ}=0$
    or $q^{MMCQ}=0$
    is at least $\frac{M_2}{1-\rho}$ for some $M_2$ independent of $\rho$ and initial joint states, given that $\rho \ge \rho^*$, for some $\rho^* < 1$. 
    Note that the time until $q^{MSJ}=0$ or $q^{MMCQ}=0$
    is a lower bound on the time until $y^{MSJ} \neq y^{MMCQ}$
\end{enumerate}

From Facts 1 and 2, we can prove Properties 1 and 2 as follows:

We call a continuous period time during which  $Y^{MSJ}(t) = Y^{MMCQ}(t)$, $Q^{MSJ}(t) \geq k+1$ and $Q^{MMCQ}(t) \geq k+1$ a \textit{good period}, and otherwise call it a \textit{bad period}. Let $y^*$ be a fixed front state, and let a $y^*$-cycle be a period that starts from the joint state $Q^{MSJ}(t)=Q^{MMCQ}(t)=0, Y^{MSJ}(t) = Y^{MMCQ}(t) = y^*$ and ends at the next same joint state when a good period happens to finish as well. By renewal reward, we have the following two equations
\begin{align}
    P(Q^{MSJ} = 0) &= \frac{E[\text{$Q^{MSJ}(t)=0$ time per $y^*$ cycle}]}{E[\text{total time per $y^*$ cycle}]}, \label{eq:property1-renewal-reward} \\ 
    P(Y^{MSJ} \neq Y^{MMCQ}) &= \frac{E[\text{$Y^{MSJ}(t)\neq Y^{MMCQ}(t)$ time per $y^*$ cycle}]}{E[\text{total time per $y^*$ cycle}]}.\label{eq:property2-renewal-reward}
\end{align}

Without out loss of generality, we assume that a cycle starts from time $0$. By Fact 1, the expected time length of a bad period conditioning on any initial joint state is at most $M_1$. 
After that, by Fact 2, we have a good period of expected length at least $\frac{M_2}{1-\rho}$, conditioned on any initial joint state. 
%In each cycle the above two types of periods will repeat for lots of times. The cycle must ends right after a second type period finishes, or in the middle of a first type period. 
Suppose in a $y^*$-cycle, we have $N$ good periods and $N$ bad periods. Then we have 
\begin{align*}
    E[\text{total time per $y^*$ cycle}] \geq \frac{M_2}{1-\rho} E[N],\\
    E[\text{$Q^{MSJ}(t)=0$ time per $y^*$ cycle}] &\leq M_1 E[N],\\
    E[\text{$Y^{MSJ}(t)\neq Y^{MMCQ}(t)$ time per cycle}] &\leq M_1 E[N].
\end{align*}
Observe that $ E[N] \geq 1$. If we further have $E[N] < \infty$, combining the above inequalities with \eqref{eq:property1-renewal-reward} and \eqref{eq:property2-renewal-reward}, we get 
\begin{align*}
    P(Q^{MSJ} = 0) &\leq \frac{M_1}{M_2}(1-\rho), \\
    P(Y^{MSJ} \neq Y^{MMCQ}) &\leq \frac{M_1}{M_2}(1-\rho).
\end{align*}

It remains to show that $E[N] < \infty$. We consider the embedded Markov chain at the end of each good period. By the definition of a $y^*$ cycle, $E[N] < \infty$ is equivalent to the fact that the expected amount of time that the embedded Markov chain returns to $(0, 0, y^*, y^*)$ is finite. 

We first show that the embedded Markov chain is positive recurrent, then show that the Markov chain has a positive probability to reach $(0, 0, y^*, y^*)$ from any joint state. Consider the Lyapunov function of the form $q - g(y)$. Both MSJ and MMCQ have negative drifts $\lambda - \rbar$ whenever $q>0$, so the continuous-time Markov chain is positive recurrent, which implies that the embedded Markov chain is also positive recurrent. 

To show that the embedded Markov chain has a positive probability to reach $(0, 0, y^*, y^*)$ from any joint state, we construct a positive-probability sample path that starts from an arbitrary joint state at the beginning of a bad period and hits $(0, 0, y^*, y^*)$ at the end of the next good period. The sample path is constructed in three steps:
\begin{itemize}
    \item Observe that at the beginning of a bad period, we have $y^{MSJ}\neq y^{MMCQ}$, so the front states of MSJ and MMCQ transition independently. There is a positive probability that before the next arrival, both front states continue to remain distinct, transition independently, and each of them have just enough completions so that $q^{MSJ} = q^{MMCQ} = 0$ and $|y^{MSJ}| = |y^{MMCQ}| = k$ (further elaborate?). 
    \item After that, consider the probability that the following sequence of events occur: first, $2k$ jobs arrive; then $k$ completions happen in both systems to clear out all jobs in the front and replacing them with freshly sampled jobs; the $k$ jobs that enter the front of both systems happen to be of the same types and in the same order. This sequence of events happen with positive probability. 
    \item After this sequence of events, we enter a good period with $y^{MSJ} = y^{MMCQ}=y$ for some $y$, and $q^{MSJ} = q^{MMCQ} = k$. By the definition of the coupling, the two systems remain identical until $q^{MSJ} = q^{MMCQ} = 0$, i.e., the end of the good period. Because the front state is an irreducible Markov chain, there is a positive-probability path from $y$ to $y^*$ with at least $k$ completions when moving on the path. When we have a suitable number of arrivals and $y^{MSJ}$ and $y^{MMCQ}$ follow that path, at the end of busy period, we have $y^{MSJ} = y^{MMCQ} = y^*$ and $q^{MSJ} = q^{MMCQ} = 0$. 
\end{itemize}



It therefore suffices to prove Facts 1 and 2. 

First Fact 1:
\begin{lemma}
    For any $\epsilon > 0$, 
    there is some constant $M_1$ 
    such that for any $\epsilon \le \rho < 1$,
    and for any joint MSJ, MMCQ state,
    the expected time until $y^{MSJ}=y^{MMCQ}$,
    $q^{MSJ} \ge k+1$, and $q^{MMCQ} \ge k+1$ is at most $M_1$.
\end{lemma}
\begin{proof}
    Call the period of time until $y^{MSJ}=y^{MMCQ}$,
    $q^{MSJ} \ge k+1$, and $q^{MMCQ} \ge k+1$
    the ``bad period.''
    We wish to show that expected length of the bad period is upper bounded by some constant $M_1$ for all $\rho \ge \epsilon$.
    
    Consider the possibility that the following sequence of events occurs:
    Over a period of 1/2 second, at least $2k+1$ jobs arrive.
    Then, over another 1/2 second, $k$ completions occur in each of the MSJ and MMCQ systems, which is sufficient to clear out every job initially present in each $y$ system and replacing them with freshly sampled jobs.
    Finally, the sampled jobs in both $y$ systems are the same, in the same order.
    
    Recall that as long as the front states of the two systems are distinct,
    their completions are independent.
    As a result, the probability of this sequence of events is positive,
    for any $\lambda$ and for any initial states $y^{MSJ},y^{MMCQ}$.
    Call the probability $pGood(\lambda, y^{MSJ},y^{MMCQ})$.
    
    Moreover, $pGood$ is monotonically increasing in $\lambda$,
    as $\lambda$ only affects the probability that at least $2k+1$ jobs arrive
    in the first half second.

    The least value of $pGood$ is achieved when $\rho = epsilon$, and hence $\lambda = \epsilon \rbar$.
    Over all $y^{MSJ},y^{MMCQ}$,
    there must be some lowest value of $pGood(\epsilon \rbar, y^{MSJ},y^{MMCQ})$.
    Call this value $pGood^*$.
    Note that for all $\lambda \ge \epsilon \rbar, y^{MSJ},y^{MMCQ}$
    \begin{align}
        pGood(\lambda, y^{MSJ},y^{MMCQ}) \ge pGood^* > 0.
    \end{align}
    In the first second, there is at least a $pGood^*$
    chance of the desired event happening and the bad period completing.
    In the next second, the same is true.
    In general, the time until the bad period completes is upper bounded by
    a geometric distribution with completion probability $pGood^*$.
    As a result the mean time until the bad period completes
    is upper bounded by $1/pGood^*$, as desired.
\end{proof}

Now fact 2:
\begin{lemma}
    There exists some constant $M_2$
    and some load $\rho^* < 1$
    such that for any $\rho \ge \rho^*$
    and
    for any joint MSJ, MMCQ state such that
    $y^{MSJ}=y^{MMCQ}$,
    $q^{MSJ} \ge k+1$, and $q^{MMCQ} \ge k+1$,
    the expected time until $q^{MSJ} = 0$ or $q^{MMCQ}=0$
    is at least $\frac{M_2}{1-\rho}$.
\end{lemma}
\begin{proof}
    Let's call the period of interest the ``good period''.
    Note that throughout the good period, $y^{MSJ}=y^{MMCQ}$.
    It therefore suffices to consider a single MSJ system, $M'$, beginning in a general state
    $y^{M'}$ and beginning with $q^{M'} = k+1$.
    The time until $q^{M'} = 0$
    is a lower bound on the length of the good period.

    Let us set up a new coupled system, $M''$.
    The $M''$ system will be initialized in a specific front state distribution to be specified later,
    and with $q^{M''}=1$.
    $M'$ and $M''$ are coupled together in the same manner as the MSJ and MMCQ system were
    previously. Note however that they are not the same systems.

    We will choose the front state distribution of the M''
    system in order to guarantee that the time until $q^{M''} = 0$
    is large in expectation.
    To do so, we will make use of the fact that the MMCQ
    system has long busy periods.

\isaac{Move to another lemma}.
    Specifically, we show that in the MMCQ,
busy periods have expected length $\Omega(\frac{1}{1-\rho})$.
To prove this, it suffices to show that
$P(Q^{MMCQ}=0) = O(1-\rho)$, and that the non-busy periods
have expected duration $\Omega(1)$.
The latter is immediate, from the fact that all transitions have expected duration $\Omega(1)$.
To prove the former, we use a linear potential function, and examine
\begin{align*}
    E[G^{MMCQ}(Q^{MMCQ} - Y^{MMCQ})] = 0 \\
    E[u(Q^{MMCQ}, Y^{MMCQ})] = \rbar - \lambda
\end{align*}
Note that $u(q, y)$ is positive if and only if $q = 0$.
Plugging in the definition of $u^{MMCQ}$,
\begin{align*}
    E[r(Y^{MMCQ})1\{Q^{MMCQ}=0\}] = \rbar - \lambda
\end{align*}
It suffices to show that $E[r(Y^{MMCQ}) | Q^{MMCQ}=0] \ge c > 0$, as this implies that
\begin{align*}
    P(Q^{MMCQ} = 0) \le \frac{\rbar - \lambda}{c} = O(1-\rho)
\end{align*}
$E[r(Y^{MMCQ}) | Q^{MMCQ}=0]\ge c$ must hold because there's some state $y$ with a positive completion rate,
and there's a positive probability of reaching that state before the next arrival.

Let $Y^{MMCQ-BP}$ denote the distribution of the front state in the MMCQ
at the start of a busy period.
By the above analysis,
the expected length of a busy period starting with $y \sim Y^{MMCQ-BP}$ and $q=1$ is
$\Omega(\frac{1}{1-\rho})$.

Let us therefore specify that the $M''$ is initialized in this exact state:
 $y \sim Y^{MMCQ-BP}$ and $q=1$.

Now, we wish to show that the expected busy period length in $M'$,
initialized in an arbitrary initial front state $y^{M'}$ and $q=k+1$,
also has long busy periods in expectation.

To prove this, let's introduce a new random object which we will couple to the
$M''$ system.
Let us introduce a very fast Poisson process,
with rate faster than $\mu^*$, the fastest transition rate in any state of $\{Y\}$.
Transitions in the $M''$ system only occur when the global Poisson increment occurs,
where with some probability sampled on each Poisson increment
a transition happens, and with the rest no transition.

To lower bound $E[B^{M'}]$, the expected busy period length in the $M'$ system,
let us consider $E[B^{M'}I\{A_1 \wedge A_2\}]$,
where $A_1$ and $A_2$ are the following two events:
\begin{enumerate}
    \item Event $A_1$: The first Poisson increment in $M''$ takes at least 1 second.
    \item Event $A_2$: During the first second $M'$ has exactly $k$ completions,
    after each of which the matching job in the front of $M''$ is sampled, resulting in $M'$ and $M''$ having identical front states $y$ and queue lengths $q=1$ after exactly $k$ completions by $A$.
\end{enumerate}
First, note that 
\begin{align}
    E[B^{M'}] \ge E[B^{M'}I\{A_1 \wedge A_2\}] = E[B^{M'} |A_1 \wedge A_2 ] P(A_1 \wedge A_2).
\end{align}
Note that $P(A_1 \wedge A_2)$ is lower bounded by a positive constant
for every $\rho \ge \epsilon$, so we can focus on $E[B^{M'} |A_1 \wedge A_2 ]$.

Note that if events $A_1$ and $A_2$ occur,
the $M'$ and $M''$ systems have the same busy period length.
As a result,
\begin{align}
    E[B^{M'} |A_1 \wedge A_2 ] = E[B^{M''} |A_1 \wedge A_2 ]
\end{align}

Note that Event $A_2$ is conditionally independent of the behavior of the $M''$ system,
given that Event $A_1$ occurs.
As a result, 
\begin{align}
    E[B^{M''} |A_1 \wedge A_2] = E[B^{M''} |A_1]
\end{align}

Notice that event $A_1$ is independent of the state of $M''$.
Conditioning on $M''$ merely increases the time of the first transition in $M''$,
without altering the future updates of $M''$ at all.
As a result,
\begin{align}
    E[B^{M''} |A_1] \ge E[B^{M''}]
\end{align}

Thus, $E[B^{M'}]$ is lower bounded by a constant multiple of $E[B(M'')]$.
Recall that by construction, $E[B^{M''}] =\Omega(\frac{1}{1-\rho})$.
We can therefore conclude that $E[B^{M'}] =\Omega(\frac{1}{1-\rho})$,
as desired.
\end{proof}





\noindent Macros and notations:\\
``MSJ'' and ``almost-$k$''\\
State variables: $Q(t)$, $Y(t)$, $Q$, $Y$, $\{Q\}_{t\geq 0}$, $\{Y\}_{t\geq 0}$, sometimes with superscripts; their realizations $q$, $y$. \\
$k$, $\lambda$, $a$, $\mu_{y,y',a}$, $\mu_y$ (or $\mu(y)$),  \\
steady-state $\pi(y)$ (or $\pi_y$)\\
instantaneous completion rate $r(\cdot)$\\
average completion rate $\rbar$\\
load $\rho$\\
discrepancy $g(y)$, number of completions up to $t$ $C_t$ \\
generator $G$, $G^{MSJ}$, $G^{always-k}$\\
completion average superscript \\
absolute value sign \\
big-O and big-Omega \\
indicator function $I\{event\}$ \\
$M_1$, $M_2$ are constants, $M'$, $M''$ are systems (?)\\
busy cycle length $B$; probability of entering a good period $pGood(\lambda, y^{MSJ}, y^{always-k})$, $pGood^*$, and other notation related to busy cycles \\
reflection $u(q, y)$, and $u = (a-q)^+$ (?) \\
$c(y)$ is a function; $C$ is a constant (?)\\
$h(q,y)$, $z(q,y)$ are functions \\
$A_1$, $A_2$ are events

~\\

\noindent Model:\\
...


\noindent Always-$k$ system: \\
Definition 1 to 6 (or only introduce concepts necessary for stating the result)\\
Theorem: expression of E[Q], see (36).\\
Proof part 1: Section 2 until (24) \\
Proof part 2: the rest of Section 2


~\\
\noindent MSJ system \\
Theorem: show that MSJ has same E[Q] expression as always-$k$\\
Lemma 1: up to the end of P4, express in terms of $Y^{MSJ}$ and indicator $Q^{MSJ}=0$\\
Lemma 2: there exists a coupling of MSJ such that $P(Q^{MSJ}=0)=O(1-\rho)$ and $P(Y^{MSJ}\neq Y^{always-k})=O(1-\rho)$. (Property 1 and Property 2)\\
Lemma 3: Fact 1\\
Lemma 4: Fact 2.




==> extra-3-3.tex <==
\hrule
This stuff was written previously, I'll combine it later



\section{Prior work}
\begin{itemize}
    \item Markov-Modulated systems
    \item MSJ.
    \item Saturated system
    \item M/G/k asymptotics
    \item Time-varying completion rates.
\end{itemize}

\section{Model}\label{sec:model}
\begin{itemize}
    \item Introduce the MSJ FCFS system, and introduce the Front/Queue concept.
    \item Introduce the Always-k system.
    \item (Mention, but not in detail, minor modifications for Limited-backfilling system)
    \item Notice that the saturated front forms a sub-Markov-chain, the ``saturated front''.
    Completion rate is only dependent on the state of this subsystem.
    \item Basic definitions: Instantaneous completion rate, time-average completion rate/throughput.
    \item Define ``Transient completions''  $g(y)$. Think of $r(Y(t)) - \rbar$ as ``transient completion rate''. Integrate to get total transient number of completions. Want a plot here.
    \item Define ``Completion-average state of saturated system''. Give formula.
    \item Define generator of a Markov chain - we will consider both the MSJ and AK generators.
\end{itemize}


% to define: the state space of saturated front, and non-saturated front
\subsubsection*{\textbf{Multiserver-job system (MSJ)}}
Consider a multiserver-job system (MSJ) with $k$ servers that serve the jobs in the First Come First Serve (FCFS) order. The jobs arrive to the system with a Poisson distribution of rate $\lambda$. Each job has a random service time with phase-type distribution and can occupy multiple servers when it is in service. We use \textit{job state} to refer to the phase and the server need of the job. \yige{define ``phase'' and ``server needs''}

\subsubsection*{\textbf{State representation of MSJ}}
The \textit{system state} of an MSJ system can be described using the state of the jobs. We split the jobs in an MSJ system into two sets: the \textit{front} and the \textit{queue}. The front consists of the $k$ jobs that arrive the earliest if there are more than $k$ jobs in the system and includes all jobs otherwise. The state of the front can be represented using a list $y$ of up to $k$ job types, where each job type indicates the server needs (the number of servers that a job occupies) and the phase of the job. If there are less than $k$ jobs in the system, we pad the vector $y$ with zeros. We denote the set of possible front states in an MSJ system as $\ysmsj$. 

The queue of an MSJ system includes all jobs that are not in the front. Because the jobs are served in the FCFS order and there are only $k$ servers, only the jobs in the front can possibly receive service. As a result, the state distribution of the jobs in the queue is equal to their initial distribution, so we can simply represent the state of the queue using its length $q$. 

In this way, an MSJ system can be studied as a continuous-time Markov chain $\{(Q^\msj(t), Y^\msj(t))\}_{t\geq 0}$, where $Q^\msj(t)$ and $Y^\msj(t)$ are the queue length and the front state of the system at time $t$. We use $(Q^{\msj}, Y^{\msj})$ to denote the steady state of the continuous-time Markov chain. \yige{$Q^{\msj}(t)$ or $Q(t)^{\msj}$? Refer to a Markov chain as $\{(Q^\msj(t), Y^\msj(t))\}_{t\geq 0}$ or $\{Q^\msj, Y^\msj\}$?}

Define the rate $\mu_{b,y,y',c}^\msj$...

\subsubsection*{\textbf{Always-$k$ system and saturated front}}
The stability and steady-state behavior of an MSJ system are closely related to a modified system called \textit{always-$k$ system}. In an always-$k$ system, apart from the usual Poisson arrivals, an additional arrival is generated if a job leaves the front while the queue is empty. \yige{The additional job is sampled from the arrival distribution} In this way, we make sure that there are always $k$ jobs in the front. We denote the set of possible front states of an always-$k$ system as $\ysak$, which is a strict subset of $\ysmsj$. 
The Markovian state of an always-$k$ system can also be represented using its queue length $Q^\ak(t)$ and its front $Y^\ak(t)$, and we denote their steady states as $Q^{\ak}$ and  $Y^{\ak}$.  \yige{Make it clear that always-$k$ is new.}

% The reason to study an always-$k$ system is that it approximates an MSJ system when the arrival rate is large enough and the MSJ system has at least $k$ jobs most of the times. Simpler system. We define a few important concepts of the always-$k$ system 

The always-$k$ system is simpler than the MSJ system because its front forms a \textit{sub-Markov-chain} whose transitions are not affected by the queue length. We call this sub-Markov-chain $\{Y^\ak(t)\}_{t\geq 0}$ the \textit{saturated front}. The saturated front determines the completions of an always-$k$ system, and thus determines the stability and the steady-state queue length of the entire always-$k$ system. We define the rate $\mu_{y, y', a}$ to be the rate that the saturated front transitions from state $y$ to $y'$ accompanied by $a$ completions, for $y, y' \in \ysak$ and $a = 0 \text{ or } 1$. \yige{change ``a'' to ``c'' }  \yige{Because the saturated front is a sub-Markov chain and is used a lot in the analysis of both MSJ and AK, can we drop the superscript of $Y^\ak$?} \yige{Write out $\mu_{y,y',a}$ explicitly?} 
\yige{``a'' always-$k$ to ``the'' always-$k$ system}
\isaac{Capitalize Always-$k$}

\subsubsection*{\textbf{Load and stability}}
Next, we define several quantities that are needed to define the \textit{load} of an MSJ system. We specify these quantities in terms of the saturated front $\{Y^\ak(t)\}_{t\geq 0}$. 
\begin{definition}
    Let $r(y)$ represent the instantaneous completion rate
    in state $y\in\ysak$:
    \begin{align*}
        r(y) = \sum_{y'\in\ysak} \mu_{y,y',1}.
    \end{align*}
\end{definition}

\begin{definition}
    Let $\pi_y$ represent the steady-state probability
    of the saturated front $\{Y^\ak(t)\}_{t\geq 0}$ being in state $y\in\ysak$:
    \begin{align*}
        \pi_y = P(Y^\ak = y).
    \end{align*} 
    \yige{$\pi_y$ and $P(Y^\ak = y)$ are synonymous?}
\end{definition}

\begin{definition}
    Let $\rbar$ represent the time-average completion rate:
    \begin{align*}
        \rbar = \sum_{y\in\ysak} \pi_{y} r(y) = E[r(Y^\ak)]. 
    \end{align*}
\end{definition}
\yige{which set of the definitions should I put into definition environments?}

Now we can define the load $\rho$ as $\rho = \lambda/\rbar$. 
 \yige{$\rho^{FCFS}$} stable if and only if $\rho < 1$. \yige{cite the correct paper}
%In the WCFS paper by Grosof et.al. \yige{cite}, it has been proved that 

\subsubsection*{\textbf{Analysis objective}}
We want to study the steady-state queue length of an MSJ system in the \textit{heavy traffic limit}, i.e., in the $\rho\to 1$ limit. Specifically, we will show that
\[
    \Ep[Q^{\msj}] = \frac{C}{1-\rho} + O(1),
\]
for some constant $C$ determined by the saturated front and independent of the load $\rho$. To specify the specific value of $C$, we will define a few more quantities. 

\subsubsection*{\textbf{Transient completion rate}}
%Next, we define several quantities that can be used to describe how the saturated front affects the steady-state queue length of an always-$k$ system. In Section~\ref{sec:results}, it turns out that the performance of an MSJ system can be quantify by the same set of quantities.
We define the \emph{transient completions} $g(y)$ from some state $y$ to be the transient additional number of completions
expected to occur in the saturated front starting from state $y$,
compared to the time-average completion rate. \yige{we call $g(y)$  ``transient completions''}
\isaac{Relative value function}
\begin{definition}
    We define transient completion rate $g(y)$ as:
    \begin{align*}
        g(y) = \int_0^\infty \Ep\left[r(Y^\ak(t)) - \rbar \middle| Y^\ak(0) = y\right] dt.
    \end{align*}
    Let $C_t$ denote the number of completions that occurs between times $0$ and $t$ in a saturated front. Then an equivalent definition of $g(y)$ is:
    \begin{align*}
        g(y) = \lim_{t \to \infty} \Ep\left[ C_t - \rbar t \middle| Y^\ak(0) = y\right].
    \end{align*}
\end{definition}
%\isaac{Need to prove $g(y)$ is well defined - use $\{Y\}$ is finite-state.}
The well-definedness of $g(y)$ comes from the fact that $\{Y^\ak(t)\}_{t\geq 0}$ has finitely many states. \yige{cite something.}

\subsubsection*{\textbf{Completion-average state}}
Next, let us define the completion-average state of the saturated front - the average state which occurs just after a completion. 
\begin{definition}
    Let $Y^e$ denote the completion-average state of $\{Y^\ak(t)\}_{t\geq 0}$:
    \begin{align*}
        \Prob(Y^e = y') = C \sum_{y\in\ysak} (\pi_y r(y)) \frac{\mu_{y,y',1}}{r(y)}
        = C \sum_{y\in\ysak} \pi_y \mu_{y,y',1}
    \end{align*}
    where $C$ is a normalization constant.
    In fact, $C = \frac{1}{\rbar}$, so this expression is actually:
    \begin{align*}
        \Prob(Y^e = y')
        = \frac{1}{\rbar} \sum_{y\in\ysak} \pi_y \mu_{y,y',1}
    \end{align*}
\end{definition}
\yige{Write $Y_d^\ak$}
% Sometimes we also need to use the completion average state of MSJ system $(Y^{\msj})^e$ given by 
% \[
%     \Prob((Y^{\msj})^e = y') = \frac{1}{\rbar} \sum_y \Prob(Y^{\msj}=y)\mu_{y,y',1}. 
% \]
% \yige{This is incorrect, the state space of MSJ front is different from the saturated front.}

% \yige{maybe define an operator that maps any random variable to their completion averages. -- NO! state space different: MSJ front state space strictly contains AK front state.}
% \begin{equation}
%     \Ep[f(Y^e)] =  \frac{1}{\rbar} \sum_{y, y'} \pi_y \mu_{y,y',1} f(y') = \Ep[ \frac{1}{\rbar} \sum_{y'} \mu_{Y,y',1} f(y')].
% \end{equation}

\subsubsection*{\textbf{Generator}}
Finally, to facilitate the proof, we consider \textit{generators} of the Markov chains under study. A generator is an operator that characterizes the infinitesimal change of a Markov chain, as defined below. 
\begin{definition}
    We define the generator of the MSJ system $G^\msj$ as an operator that acts on any real-valued function $f(q, y)$ and gives
    \begin{align*}
        G^\msj f(q, y) = \lim_{s \to 0} \frac{1}{s} \Ep\left[f(Q^\msj(s)), Y^\msj(s)) - f(q,y)\middle|Q^\msj(0)=q, Y^\msj(0) = y\right].
    \end{align*}
    Similarly, we define the generator of the always-$k$ system $G^\ak$ as an operator that acts on any real-valued function $f(q,y)$ and gives 
    \begin{align*}
        G^\ak f(q, y) = \lim_{s \to 0} \frac{1}{s} \Ep\left[f(Q^\ak(s), Y^\ak(s)) - f(q, y)\middle|Q^\ak(0)=q, Y^\ak(0) = y\right].
    \end{align*}
\end{definition}

The generators for the MSJ and always-$k$ systems can be explicitly written as 
\begin{equation}
    G^\ak f(q,y) = \lambda \left(f(q+1, y) - f(q, y) \right) + \sum_{\substack{y'\in\ysak,\\ a\in\{0,1\}}} \mu_{y, y', a} \left(f((q-a)^+, y') - f(q, y)\right).
\end{equation}
\begin{equation}
    \begin{aligned}
        G^{\msj} f(q, y) = \begin{cases}
            G^{\ak} f(q, y) & q > 0 \\
            0 & |y| < k-1 \\
            (\text{arrivals only}) & |y| = k-1 \\
            (\text{anything}) & |y| = k, q = 0
        \end{cases}
    \end{aligned}
\end{equation}
\yige{Here we need $\mu_{y,y',a}$ in the expression of $G^\msj f(q,y)$ when $q=0$.}
\isaac{This expression for $G^\msj$ is wrong - correct should look more like the AK expression.}


Later proofs will rely on the following relationship:
for any suitable function of the form $f(q, y)$, we have 
\begin{align}
    \Ep[G^\msj f(Q^\msj, Y^\msj)] &= 0, \label{eq:msj-bar}\\
    \Ep[G^\ak f(Q^\ak, Y^\ak)] &= 0. \label{eq:ak-bar}
\end{align}
\yige{State a sufficient condition for our $f$ to satisfy the above relation}
%\yige{Maybe write out the specific expression of a generator, and state the drift condition only for the specific class of $f(q,y) = (q-g(y))^2 + h(y)$ under use to avoid repetition and stating unnecessary technical conditions. (?)}

\subsubsection*{\textbf{Other notations}}
Big-O notation, only about $\rho$; equal in distribution $\overset{d}{=}$




\section{Main results}\label{sec:results}
\begin{itemize}
    \item State the main theorem.
    \item Give a proof sketch of how we're going to prove it.
    Basic idea: 1. AK has this asymptotic behavior. 2. MSJ and AK have same asymptotic behavior.
    We prove 1 using a generator approach, 2 is quite technically involved.
    To prove 2, we make use of a coupling. We make use of AK's long busy periods.
\end{itemize}

\begin{theorem}[Queue length asymptotics of multiserver-job systems]\label{thm:msj-queue-length}
    In a multiserver-job system, the expected queue length in steady state satisfies
    \begin{equation}\label{eq:msj-queue-length}
        \Ep[Q^{\msj}] =  \frac{\Ep[g(Y^e)] + 1 }{1 - \rho} + O(1).
    \end{equation}
\end{theorem}

Now we give a proof sketch of Theorem~\ref{thm:msj-queue-length}. The proof sketch consists of two steps: we first figure out the queue length of an always-$k$ system, then show that an MSJ system has similar queue length asymptotics in the heavy traffic limit of $\rho \to 1$. The second step is quite technically involved and we leave most of the details to Section~\ref{sec:proofs}.
\subsubsection*{\textbf{Step 1}}
In the first step, we focus on the always-$k$ system and show that it satisfies \eqref{eq:msj-queue-length}, i.e.
\begin{align}
    \Ep[Q^{\ak}] = \frac{\Ep[g(Y^e)] + 1}{1-\rho} + O(1).
\end{align}
We prove this using a generator approach. We calculate $G^\ak f(q, y)$ with $f(q,y) = \frac{1}{2}(q-g(y))^2$, giving
\begin{equation}\label{eq:G-ak-f}
    G^\ak f(q,y) = (\lambda - \rbar) q - c(y) + O(1) \cdot \indic_{q=0},
\end{equation}
where $c(y)$ is a function that only depends on $y$. We choose $f(q,y) = \frac{1}{2}(q-g(y))^2$
in order to ensure that $G^\ak f(q,y)$ separates into a term dependent only on $q$ and a term dependent only on $y$.

Using the condition that $\Ep[G^{\ak} f(Q^{\ak}, Y^{\ak})]= 0$, we have
\begin{align}
    \label{eq:generator-steady}
    0 &= (\lambda - \rbar) \Ep[Q^\ak] - \Ep[c(Y^\ak)] + O(1)\cdot \Prob(Q^\ak=0).
\end{align}
We show that $\Ep[c(Y^\ak)] = \rbar~(\Ep[g(Y^e)] + 1)$ and that $\Prob(Q^\ak=0) = 1-\rho$.

We divide \eqref{eq:generator-steady} by $\rbar - \lambda = \rbar (1-\rho)$ to get 
\[
    \Ep[Q^\ak] = \frac{\Ep[c(Y^\ak)]}{\rbar - \lambda} + O(1) \cdot \frac{\Prob(Q^\ak =0)}{\rbar - \lambda} = \frac{\Ep[g(Y^e)] + 1}{1-\rho} + O(1).
\]
\yige{include more calculation details in \eqref{eq:G-ak-f}?} \yige{This $c(y)$ corresponds to $c'(y)$ in the first draft of proofs.} 

\subsubsection*{\textbf{Step 2}}
We prove that MSJ and always-$k$ systems have similar asymptotic behaviors. 
% \begin{align}
%     \Ep[Q^{\msj}] &= \Ep[Q^{\ak}] + O(1) = \frac{\Ep[g(Y^e)] + 1}{1-\rho} + O(1),
% \end{align}
We observe that the generator of $\msj$ and $\ak$ are identical except when $q = 0$, so using the same test function $f(q, y) = \frac{1}{2}(q - g(y))^2$ \isaac{Test function only valid for $y \in Y^{AK}$. Define $f^\msj$.}, we can get a formula almost identical to \eqref{eq:G-ak-f}:
\begin{equation}\label{eq:G-msj-f}
    G^\msj f(q,y) = (\lambda - \rbar) q - c(y) + O(1) \cdot \indic_{q=0},
\end{equation}
whose only difference with \eqref{eq:G-ak-f} is that the $O(1)$ represents a different expression. Using the condition that $\Ep[G^\msj f(Q^\msj, Y^\msj)] = 0$, we have
\[
    0 = (\lambda - \rbar)\Ep[Q^\msj] - \Ep[c(Y^\msj)] + O(1)\cdot \Prob(Q^\msj = 0).
\]
We will exhibit a coupling between an MSJ system and an always-$k$ system under which $\Prob(Y^\msj \neq Y^{\ak}) = O(1-\rho)$, and show that $\Prob(Q^\msj = 0) = O(1-\rho)$. As a result, we have
\begin{align*}
    0 &= G^{\msj} f(Q^{\msj}, Y^{\msj}) = (\lambda - \rbar)\Ep[Q^{\msj}] - \Ep[c(Y^{\ak})] + O(1-\rho), \\
    E[Q^{\msj}] &= \frac{\Ep[c(Y^{\ak})]}{\rbar - \lambda} + O(1) = \frac{1+\Ep[g(Y^e)]}{1-\rho} + O(1).
\end{align*}
\isaac{Notation $Y^e$ is not very clear because unclear whether AK or MSJ system - write $Y^{AK}_d$ instead.}

The coupling is constructed as below: we let the two systems have Poisson arrivals at the same time. If their front states $y^\msj$ and $y^\ak$ are the same and $q>0$, we let their next completions and transitions to be the same; otherwise, we let their next completions and transitions be independent. \yige{when $y^\msj = y^\ak$ and $q=0$, they have independent completion times}

We show that the two systems starting from any initial states will ``mix''\yige{merge} in $O(1)$ time, i.e., having $y^\msj = y^\ak$, and remain so until $q^\msj$ or $q^\ak$ hits zero again. Using another coupling argument, we show that the time until  $q^\msj$ or $q^\ak$ hits zero is $\Omega(1/(1-\rho))$. % Roughly speaking, long ``busy periods'', during which $q=0$ or $y^\msj \neq y^\ak$ only last for a short fraction of time at the beginning of the busy period. 
\yige{to complete}

\yige{refer to the lemmas; incorporate the outline of Section 5 and the statement of the lemmas}



\section{Proof of main theorem}\label{sec:proofs}
\begin{itemize}
    \item Lemma 1: Mean queue length in AK system has the right asymptotics. Uses generator approach.
    \item Discuss main coupling - between AK system and MSJ system.
    \item Lemma 2: Enter coupling (main coupling) in constant expected time. Direct.
    \item Lemma 3: Remain coupled (main coupling) and nonempty for long period of time. Mostly direct, use long busy period in AK system (based on Lemma 1). Discuss secondary coupling.
    \item Lemma 4: Almost never empty and almost always coupled (main coupling). Proof: use renewal reward, use Lemma 2 and 3.
    \item Theorem: Using the generator approach for the MSJ system, and using the ``almost never empty`` and ``almost always coupled'' results, we show that the MSJ system has the same asymptotics as the AK system, which are the right asymptotics (using Lemma 1).
\end{itemize}

\begin{lemma}[Queue length asymptotics of always-$k$ systems]\label{lem:ak-queue-length}
    In an always-$k$ system, the expected queue length in steady state satisfies
    \begin{equation}\label{eq:ak-queue-length}
        \Ep[Q^\ak] = \frac{E[g(Y^e)] + 1 }{1 - \rho} + O(1).
    \end{equation}
\end{lemma}


The coupling is constructed as below: we let the two systems have arrivals at the same time. If their front states $y^\msj$ and $y^\ak$ are the same and $q>0$, we let their next completions and transitions to be the same; otherwise, we let their next completions and transitions be independent. \yige{repetitive paragraph}


\begin{lemma}
    From any joint MSJ, always-$k$ state, under the coupling above,
    the expected time until $y^{\msj}=y^{\ak}$, $q^{\msj} \ge k+1$, and $q^{\ak} \ge k+1$
    is at most $M_1$ for some $M_1$ independent of $\rho$ and initial joint states,
    given that $\epsilon \le \rho < 1$.
\end{lemma}



\begin{lemma}
    From any joint MSJ, always-$k$ state such that
    $y^{\msj}=y^{\ak}$, $q^{\msj} \ge k+1$, and $q^{\ak} \ge k+1$, the expected time until $q^{\msj}=0$
    or $q^{\ak}=0$
    is at least $\frac{M_2}{1-\rho}$ for some $M_2$ independent of $\rho$ and initial joint states, given that $\rho \ge \rho^*$, for some $\rho^* < 1$. 
\end{lemma}
Note that the time until $q^{\msj}=0$ or $q^{\ak}=0$ is a lower bound on the time until $y^{\msj} \neq y^{\ak}$.


\begin{lemma}
    In a multiserver-job system, for any $\epsilon \le \rho < 1$, we have the following two properties:
    \begin{enumerate}
    \item Property 1: $P(Q^{\msj}=0) = O(1-\rho)$
    \item Property 2: $P(Y^{\msj} \neq Y^{\ak}) = O(1-\rho)$.
    \end{enumerate}
    where property 2 holds under the coupling specified above.
\end{lemma}



\begin{proof}[Proof of Theorem~\ref{thm:msj-queue-length}]
    to-do
\end{proof}



\subsection{Some basic facts that need to appear at certain points} 
Note that $\Ep[g(Y^\ak)] = 0$, because $Y^\ak(s) \overset{d}{=} Y^\ak$ for all $s$, and so $\Ep[r(Y(s))] = \rbar$.

\isaac{A useful set of linear equations for solving for $g(y)$, up to an additive constant:}
\begin{align*}
    \isaac{\qquad g(y) = \frac{r(y) - \rbar}{\mu(y)} + \sum_{y'} g(y') \frac{\mu_{y,y'}}{\mu(y)} \qquad}
\end{align*}


A generator has the following relationship with relative value function \isaac{For example, $G^\ak g(y) = \rbar - r(y)$.}





\section{Empirical}
Plots of MSJ FCFS compared to theoretical analysis.

\section{Discussion}
Other applications of this approach. 
\begin{itemize}
    \item Other MSJ policies that are finite-skip. Example: FCFS + k-job front backfilling. Framed paper around FCFS, but acually lots of MSJ policies it would apply to.
    \item Exogeneously influenced completion rates (MMCQ). Ex: Suppose we have server with time-varying speeds due to outside contention. Lemma 1 alone.
\end{itemize}
\section{Conclusion}




\input{draft-of-proofs.tex}




==> extra.tex <==
\iffalse
Now, let us define a ``coupled busy period''
to be an interval where $Q > 0$ and
$Y^{MSJ} = Y^{MMCQ}$.
We will show that the expected time between
coupled busy periods is $O(1)$
and the expected length of a coupled busy period is $\Omega(\frac{1}{1-\rho})$.
This implies that the time spend outside of a coupled busy period is $O(1-\rho)$,
which implies our two desired facts.

First, to show that the expected time between coupled busy periods is $O(1)$,
note that from an arbitrary state,
the is a positive probability of coupling in a busy state in $O(1)$ time,
via $2k$ arrivals and $k$ completions.

Now, we are ready for the meat of the proof:
Showing that coupled busy periods
have expected length $\Omega(\frac{1}{1-\rho})$.

First, we show that in the MMCQ,
busy periods have length $\Omega(\frac{1}{1-\rho})$.
To prove this, it suffices to show that
$P(Q^{MMCQ}=0) = O(1-\rho)$.
To prove this, we use a linear potential function, and examine
\begin{align*}
    E[G^{MMCQ}(Q^{MMCQ} - Y^{MMCQ})] = 0 \\
    E[u(Q^{MMCQ}, Y^{MMCQ})] = \rbar - \lambda
\end{align*}
Note that $u(q, y)$ is positive if and only if $q = 0$.
Plugging in the definition of $u^{MMCQ}$,
\begin{align*}
    E[r(Y^{MMCQ})1\{Q^{MMCQ}=0\}] = \rbar - \lambda
\end{align*}
It suffices to show that $E[r(Y^{MMCQ}) | Q^{MMCQ}=0] \ge c > 0$, as this implies that
\begin{align*}
    P(Q^{MMCQ} = 0) \le \frac{\rbar - \lambda}{c} = O(1-\rho)
\end{align*}
$E[r(Y^{MMCQ}) | Q^{MMCQ}=0]\ge c$ must hold because there's some state $y$ with a positive completion rate,
and there's a positive probability of reaching that state before the next arrival.


TODO: Significant rewrites, see photo.

\yige{The content starting from "coupled busy period" can be replaced by ...}


\begin{definition}
    Define $BP(y)$ as the length of a busy period of a MMCQ system (or equivalently, a MSJ system) when it is started from state $y$. Formally,
    \begin{equation}
        BP(y) = \inf\{t: Q(t)=0| Y(0) = y, Q(0) = 1\}.
    \end{equation}
\end{definition}

Let $Y^{MMCQ-BP}$ denote the state distribution sampled at times when a MMCQ system begins a busy period. Let $Y^{MSJ-BP}$ denote the state distribution sampled at times when a MSJ system begins busy period. 

\begin{definition}
    Given the coupling defined above, define $GoodBP(y, y')$
    to be the amount of time prior to either the MSJ or MMCQ system emptying
    such that $Y^{MSJ}=Y^{MMCQ}$, given that MSJ starts from $(k+1,y)$ and MMCQ starts from $(1,y')$.
\end{definition}

We have
\begin{equation}
    E[BP(Y^{MMCQ-BP})] = \Omega(\frac{1}{1-\rho}).
\end{equation}

We want to show that 
\begin{equation}
    \label{eq:good-bp}
    E[GoodBP(y, y')] \geq  \epsilon\cdot E[BP(y')],
\end{equation}
for some fixed $\epsilon>0$, dependent on the characteristics of the MSJ system but not on $\rho$ and any $y, y'$, which implies that
\begin{equation}
    E[GoodBP(Y^{MSJ-BP}, Y^{MMCQ-BP})] \geq  \epsilon \cdot  E[BP(Y^{MMCQ-BP})] = \Omega(\frac{1}{1-\rho}).
\end{equation}

\isaac{Busy period starts least $k+1$}
Note that
\begin{align}
    E[BP(y)] \ge E[GoodBP(y, y')] \qquad \forall y'
\end{align}
so this is sufficient to prove that
\begin{align}
    E[BP(Y^{MSJ-BP})] = \Omega(\frac{1}{1-\rho})
\end{align}

\isaac{Coupling 1: Long-term coupling}

From this, we argue that probability that the MSJ system is nonempty is $O(1-\rho)$,
and that the probability that the MSJ and MMCQ systems are not coupled is $O(1-\rho)$.

To prove this, not that the time spent not busy per busy cycle is $O(1)$,
by the following geometric bounding argument:
From a given MSJ state, there is a nonzero probability $p$ that after 1 second,
the system is busy. Therefore, the time spent nonbusy is bounded by $Geo(p)$.
$p$ is not dependent on the MSJ state, or on how close $\rho$ is to 1.
The same argument also shows that the time spent not coupled
per busy cycle is $O(1)$.

Now, we use a renewal reward argument to show that the probability that our
system is empty or uncoupled is $O(1)$.
Our renewal points are times when the MSJ and MMCQ systems are each in specified states.
(Lyapunov drift here $q-g(y)$).

\isaac{Proof uses Coupling 2, short-term, starts when system $A$ has $k+1$ jobs}

Now let's show \eqref{eq:good-bp} is true.
GoodBP is defined with respect to two systems, one beginning in state $y$, one in state $y'$.
Above, these were described as an MSJ and MMCQ system,
but the two have identical dynamics throughout the period when both systems are busy,
so the distinction is irrelevant.

Call these systems $A$ and $C$.
We'll think about transition in $C$ happening slightly differently.
Imagine there is a very fast global Poisson process,
with rate faster than $\mu^*$, the fastest transition rate in any state of $\{Y\}$.
Transitions in $C$ can only occur when the global Poisson occurs,
where with some probability sampled on each Poisson beat
a transition happens, and with the rest no transition.
The global Poisson rate is constant.
We will condition on two events:
\begin{enumerate}
    \item The first Poisson beat in $C$ takes at least 1 second.
    \item During the first second $A$ has exactly $k$ completions,
    after each of which the matching job in $C$ is sampled, resulting in $A$ and $C$ being coupled after exactly $k$ completions by $A$.
\end{enumerate}

Expected good busy period length
is at least $P(\text{Both happen})$
times $E[BP^C | \text{Both happen}]$.
The probability $P(\text{Both happen})$ is lower bounded by a positive constant for all $\rho$, by the standard probablistic argument.

As for the expectation $E[BP^C | \text{Both happen}]$, 
Item 2 are conditionally independent of the events in $C$ after the first 1 second.
As a result, $E[BP^C | \text{Both happen}] = E[BP^C | \text{Slow first Poisson beat (1)}]$.
Having a slow first Poisson beat is independent of the initial state of $C$,
and merely increases the time to the first transition in $C$ without changing any distributions.
As a result, $E[BP^C | \textit{Slow first Poisson beat}] \ge E[BP^C]$
as desired.
\fi

==> leftovers.tex <==
\isaac{TODO: outlines of each section, which should go at the top of each section.}
\iffalse

\subsubsection{MSJ and Always-$k$ system have same asymptotic mean response time}
We will now prove \cref{thm:msj-response-time}, our main theorem:

\begin{reptheorem}{thm:msj-response-time}
    In the multiserver-job system, the expected response time in steady state satisfies
    \begin{align}
        E[T^{MSJ}] = \frac{1}{\lambda^*} \frac{1+\Delta(Y^{Sat}_d, Y^{Sat})}{1-\frac{\lambda}{\lambda^*}}+O_\lambda(1)
    \end{align}
\end{reptheorem}

To prove that MSJ and always-$k$ systems have the same asymptotic behavior,
we again start with a generator approach.
The updates of the MSJ and Always-$k$ systems are identical except whenever $q > 0$. We therefore use the same test function $f(q, y) = \frac{1}{2}(q - g(y))^2$ whenever $y \in Y^{AK}$. Doing so, we get a formula almost identical to \eqref{eq:G-ak-f-main}:
\begin{equation}\label{eq:G-msj-f-main}
    G^\msj \circ f(q,y) = (\lambda - X^{Sat}) q - c(y) + O_\lambda(1) \cdot \indic_{q=0}.
\end{equation}
Note that $c(y)$ is the same function which appears in \eqref{eq:G-ak-f-main}.
Using the condition that \qquad \qquad \, $\Ep[G^\msj\circ f(Q^\msj, Y^\msj)] = 0$, we have
\begin{align}
\label{eq:generator-msj-steady-main}
    0 = (\lambda - X^{Sat})\Ep[Q^\msj] - \Ep[c(Y^\msj)] + O(1)\cdot \Prob(Q^\msj = 0).
\end{align}
Comparing \eqref{eq:generator-msj-steady-main} to \eqref{eq:generator-steady-main}, we see that the two equations are identical,
except that $Y^\ak$ and $Q^\ak$ have been replaced by $Y^\msj$ and $Q^\msj$.
To complete the proof, we will show that $Y^\msj$ and $Y^\ak$
are similar distributions,
and that $P(Q^\msj = 0)$ is similar to $P(Q^\ak = 0)$.
This is the hardest technical step of the paper.

To make this formal, in \cref{sec:coupling} we design a coupling between the MSJ system and the Always-$k$ system.
We show in \cref{lem:quick-merge} that, under our coupling, the two systems starting from any initial states will merge in $O_\lambda(1)$ time, i.e., have $y^\msj = y^\ak$,
and remain merged until $q^\msj$ or $q^\ak$ next reaches zero.
We refer to this period of time as a "busy period".
In \cref{lem:long-busy}, using another coupling argument, we show that the
expected duration of this busy period is $\Omega_\lambda(1/(1-\frac{\lambda}{X^{Sat}}))$.
In \cref{lem:tight-coupling}, using a renewal-reward argument,
we then show that 
$\Prob(Y^\msj \neq Y^{\ak}) = O_\lambda(1-\frac{\lambda}{X^{Sat}})$.
We also use the coupling to show that $\Prob(Q^\msj = 0) = O_\lambda(1-\frac{\lambda}{X^{Sat}})$.

Finally, in \cref{sec:main-proof}, we combine these lemmas with \eqref{eq:generator-msj-steady-main} to show that
\begin{align*}
    0 &= (\lambda - X^{Sat})\Ep[Q^{\msj}] - \Ep[c(Y^{\ak})] + O_\lambda(1-\frac{\lambda}{X^{Sat}}) \\
    \implies E[Q^{\msj}] &= \frac{\Ep[c(Y^{\ak})]}{X^{Sat} - \lambda} + O_\lambda(1) =
    \frac{1+\Delta(Y^{Sat}_d,Y^{Sat})}{1-\frac{\lambda}{X^{Sat}}} + O_\lambda(1).
\end{align*}
Applying Little's law and the fact that $\lambda^* = X^{Sat}$ completes the proof of \cref{thm:msj-response-time}.
\fi

==> lemma_statements.tex <==
\subsection{Lemma on Ak system}
\isaac{Prove generator applied to Delta}
\isaac{AK system asymptotics}

\begin{lemma}
    \begin{equation}
        G^\ak \circ \Delta(y, Y^{Sat}) = X^{Sat} - X^{\sat}_{y}
    \end{equation}
\end{lemma}

\begin{lemma}
    Let $f(q,y)$ be a real-valued function of the state of the Always-$k$ system, then
    \begin{equation}
        G^\ak \circ f(q,y) =  \lambda \left(f(q+1, y) - f(q, y) \right) + \sum_{\substack{y'\in\ysak,\\ a\in\{0,1\}}} \mu_{y, y', a} \left(f((q-a)^+, y') - f(q, y)\right).
    \end{equation}
\end{lemma}

\begin{theorem}[Mean response time asymptotics of always-$k$ systems]\label{thm:ak-response-time}
    In the Always-$k$ system, the expected response time in steady state satisfies
    \begin{equation}\label{eq:ak-response-time}
        \Ep[T^\ak] = \frac{1}{\lambda^*} \frac{1+\Delta(Y^{Sat}_d, Y^{Sat})}{1-\frac{\lambda}{\lambda^*}}+O_\lambda(1).
    \end{equation}
\end{theorem}

\subsection{Introduce main coupling, Coupling Lemmas}
\label{sec:coupling}
\isaac{Lemma: Merge in $O(1)$ time.}
\isaac{Lemma: Remain merged and nonempty for long time. Uses secondary coupling}
\isaac{Lemma: Almost never empty, almost always merged. Renewal reward.}

To show that the Always-$k$ system and the Multiserver-job system have identical asymptotic mean response time, we define a coupling of the two systems as below. We let the arrivals of the two systems happen at the same time. We couple the transitions of their front states based on their joint state $(q^\msj, y^\msj, q^\ak, y^\ak)$: if $y^\msj=y^\ak$ and $q^\msj, q^\ak>0$, we let them have the same transitions of the front states (this means the completions happen at the same time, and when the completion happens, the the same type of jobs are leaving the system and entering the front); otherwise, we let their transitions of the front states be independently sampled.



\begin{lemma}[Quick merge]
    \label{lem:quick-merge}
    From any joint MSJ, always-$k$ state, under the coupling above,
    the expected time until $y^{\msj}=y^{\ak}$, $q^{\msj} \ge k+1$, and $q^{\ak} \ge k+1$
    is at most $M_1$ for some $M_1$ independent of the arrival rate $\lambda$ and initial joint states,
    given that $\epsilon \le \lambda < \lambda^*$.
\end{lemma}

\begin{lemma}[Long busy period]
    \label{lem:long-busy}
    From any joint MSJ, always-$k$ state such that
    $y^{\msj}=y^{\ak}$, $q^{\msj} \ge k+1$, and $q^{\ak} \ge k+1$, the expected time until $q^{\msj}=0$
    or $q^{\ak}=0$
    is at least $\frac{M_2}{1-\rho}$ for some $M_2$ independent of the arrival rate $\lambda$ and initial joint states, given that $\lambda \ge \lambda^*$, for some $\lambda^* < 1$. 
\end{lemma}
Note that the time until $q^{\msj}=0$ or $q^{\ak}=0$ is a lower bound on the time until $y^{\msj} \neq y^{\ak}$.

\begin{lemma}[Tight coupling]
    \label{lem:tight-coupling}
    In the MSJ system, for any $\epsilon > 0$ and for any $\lambda$ s.t. $\epsilon \le \lambda < \lambda^*$, we have the following two properties:
    \begin{enumerate}
    \item Property 1: $P(Q^{\msj}=0) = O_\lambda(1-\frac{\lambda}{\lambda^*})$
    \item Property 2: $P(Y^{\msj} \neq Y^{\ak}) = O_\lambda(1-\frac{\lambda}{\lambda^*})$.
    \end{enumerate}
    where property 2 holds under the coupling specified above.
\end{lemma}


\subsection{Proof of \cref{thm:msj-response-time}}
\label{sec:main-proof}
\isaac{Generator and lemmas, same asymptotics as Ak system.}
\isaac{Convert to response time, show that $O_\lambda(\frac{1}{\lambda})= O(1)$.}

\begin{lemma}
    Let $f(q,y)$ be a real-valued function of the state of the MSJ system, then
    \begin{equation}
        G^\msj \circ f(q,y) =  \lambda \left(f(q+1, y) - f(q, y) \right) \indic_{\{y\in\ysak\}} + \sum_{\substack{y'\in\ysmsj,\\ a\in\{0,1\}}} \mu_{\indic_{\{q>0\}}, y, y', a} \left(f((q-a)^+, y') - f(q, y)\right).
    \end{equation}
    \isaac{where $\mu_{1, y, y', a}=\mu_{y,y',a}$, and $\mu_{0, y, y', a}$ is to be defined in the model section.}
\end{lemma}

\begin{reptheorem}{thm:msj-response-time}
    In the multiserver-job system, the expected response time in steady state satisfies
    \begin{align}
        E[T^{MSJ}] = \frac{1}{\lambda^*} \frac{1+\Delta(Y^{Sat}_d, Y^{Sat})}{1-\frac{\lambda}{\lambda^*}}+O_\lambda(1)
    \end{align}
\end{reptheorem}

